Conversational Assistants in Knowledge-Intensive Contexts: An Evaluation of LLM- versus Intent-based Systems

Conversational Assistants (CA) are increasingly supporting human workers in knowledge management. Traditionally, CAs respond in specific ways to predefined user intents and conversation patterns. However, this rigidness does not handle the diversity of natural language well. Recent advances in natural language processing, namely Large Language Models (LLMs), enable CAs to converse in a more flexible, human-like manner, extracting relevant information from texts and capturing information from expert humans but introducing new challenges such as ``hallucinations''. To assess the potential of using LLMs for knowledge management tasks, we conducted a user study comparing an LLM-based CA to an intent-based system regarding interaction efficiency, user experience, workload, and usability. This revealed that LLM-based CAs exhibited better user experience, task completion rate, usability, and perceived performance than intent-based systems, suggesting that switching NLP techniques can be beneficial in the context of knowledge management.

==> tools.tex <==
\usepackage{acro}

\DeclareAcronym{km}{
  short=KM,
  long=knowledge management,
}

\DeclareAcronym{kms}{
  short=KMS,
  long=knowledge management system,
}

\DeclareAcronym{is}{
  short=IS,
  long=information system,
}

\DeclareAcronym{nlp}{
  short=NLP,
  long=natural language processing,
}

\DeclareAcronym{llm}{
  short=LLM,
  long=large language model,
}

\DeclareAcronym{ux}{
  short=UX,
  long=user experience,
}

\DeclareAcronym{ai}{
  short=AI,
  long=artifical intelligence,
}

\DeclareAcronym{rag}{
  short=RAG,
  long=retrieval augmented generation,
}

\DeclareAcronym{sus}{
  short=SUS,
  long=system usability scale,
}

\DeclareAcronym{ueq}{
  short=UEQ,
  long=user experience questionnaire,
}

\DeclareAcronym{tlx}{
  short=NASA-TLX,
  long=NASA task load index,
}

\DeclareAcronym{sd}{
  short=SD,
  long=standard deviation,
}

\DeclareAcronym{hci}{
  short=HCI,
  long=human-computer interaction,
}
